SPADE: Sparse Pillar-based 3D Object Detection Accelerator for Autonomous Driving

3D object detection using point cloud (PC) data is essential for perception pipelines of autonomous driving, where efficient encoding is key to meeting stringent resource and latency requirements. PointPillars, a widely adopted bird's-eye view (BEV) encoding, aggregates 3D point cloud data into 2D pillars for fast and accurate 3D object detection. However, the state-of-the-art methods employing PointPillars overlook the inherent sparsity of pillar encoding where only a valid pillar is encoded with a vector of channel elements, missing opportunities for significant computational reduction. Meanwhile, current sparse convolution accelerators are designed to handle only element-wise activation sparsity and do not effectively address the vector sparsity imposed by pillar encoding. In this paper, we propose SPADE, an algorithm-hardware co-design strategy to maximize vector sparsity in pillar-based 3D object detection and accelerate vector-sparse convolution commensurate with the improved sparsity. SPADE consists of three components: (1) a dynamic vector pruning algorithm balancing accuracy and computation savings from vector sparsity, (2) a sparse coordinate management hardware transforming 2D systolic array into a vector-sparse convolution accelerator, and (3) sparsity-aware dataflow optimization tailoring sparse convolution schedules for hardware efficiency. Taped-out with a commercial technology, SPADE saves the amount of computation by 36.3--89.2\% for representative 3D object detection networks and benchmarks, leading to 1.3--10.9$\times$ speedup and 1.5--12.6$\times$ energy savings compared to the ideal dense accelerator design. These sparsity-proportional performance gains equate to 4.1--28.8$\times$ speedup and 90.2--372.3$\times$ energy savings compared to the counterpart server and edge platforms.

==> Sections/3_method1.tex <==

\section{Sparse Pillar Network (SP-Net)}
\label{sec:sp-net}

Although extensive sparsity exists in pillar encoding, most pillar-based neural networks have ignored performance improvement from it~\cite{wang2020pillar, zhou2020end, sun2020scalability, li2021lidar, shi2022pillarnet,yin2021center}. Up to our knowledge, \cite{vedder2021sparse} is the only attempt that employ sparse convolution for expediting execution of PointPillars. Following the prior voxel-based sparse convolution models, Sparse PointPillars~\cite{vedder2021sparse} (SPP) modified the original model structure of PointPillars by replacing Conv2D with stride one and two with sub-manifold convolution (SubM-Conv) and 2D sparse convolution, respectively. In this modification, SubM-Conv maintains the sparsity of the input pillars since it ignores the dilation effect of convolution. Also, sparse convolution increase the number of output pillars due to dilation, its dilation effect is small as it replaces Conv2D with stride two. In other words, SPP maintains sparsity of pillars by strictly avoiding dilation effect of sparse convolution. Such attempts result in improved 3D object detection speed~\cite{vedder2021sparse}.

However, we discover that the dilation effect of convolution plays a critical role in achieving high accuracy of 3D object detection. As an illustration of the issue, [Fig. YY] exhibits the heat maps of active pillars across the layers. The top row is the heat maps retrieved from SPP, in which the white boxes indicate the ground-truth location of objects for the given point cloud input. As the heat maps show, the location of active pillars in SPP are initially concentrated near the sensor, and their locations are mostly fixed throughout the layers. Note that some of the ground-truth locations are covered by few active pillars, especially for the objects far from the sensor. Since the active pillars little propagate in SPP, these crudely covered ground-truth locations remain lack of active pillars. Therefore, SPP cannot properly identify the objects for those rarely-covered locations and suffer significant accuracy degradation, as shown in [Table YY].  

The key insight obtained from the observation of heat maps is that active pillars should propagate features around. To this end, we propose an intuitive yet effective sparse pillar network (SP-Net). The overall structure of SP-Net is described in [Fig. YY] (b). Different from SPP, SP-Net employs only sparse convolution (instead of SubM-Conv) to allow dilation across the layers, but dynamically prune the unimportant pillars so that the overall sparsity is maintained. Noting that bias addition artificially increase the pillar density, we exclude bias-add from sparse convolution and take Batchnorm only for the sparse points. The output pillars of sparse convolution are compared with a pre-determined threshold to zero out unimportant pillars. Since this selection of active pillars depend on the representative value of each pillar vector, the sparsity can be automatically adjusted for point cloud of each frame. 

To determine a proper threshold for all sparse convolutions, we develop a pruning-aware fine-tuning algorithm, as described in [Fig. YY] (c). First, we regularize the 3D object detection network to tune the network more friendly to pillar pruning. Note that pillar pruning requires zero-out of an entire pillar vector. Therefore, we adopt Group Lasso ([REF]) on each pillar vector to suppress the magnitude of vector elements altogether, as follows:
\begin{equation}
\begin{aligned}
loss_{GroupLasso}&=\alpha\sum_{l=1}^{L}(\sum_{p_l=1}^{P_l}||X_{P_l,:}^l||_{g})\\
||X_{p_l,:}||_{g}&=\sqrt{\sum_{c=1}^{C_{p_l}}(X_{p_l,c})^{2}}
\end{aligned}
\label{eq:group_lasso}
\end{equation}
where, $\alpha$ is the temperature, $l$ is the number of the layer, $p$ is the non-empty pillars, $X$ is the activation of the layer, and $C$ is the channel of activation.
Thus, elements of unimportant pillars would move close to zero and become more pruning friendly. Then, we apply pruning and perform fine-tuning of weight parameters to be adjusted for the pruned activation. Pruning thresholds for all the sparse convolutions are retrieved after fine-tuning for a small number of epochs. % regularization-pruning-fine-tuning can be done altogether.
In inference time, the retrieved pruning thresholds are incorporated in SP-Net to dynamically prune the output pillars of sparse convolution. Our pruning-aware fine-tuning is distinctive from prior activation pruning techniques for 2D convolutional neural networks in that the conventional activation pruning relies on element-wise activation sparsity due to ReLU activation function, whereas our pruning is based on the inherent structured activation sparsity of pillars.

The advantage of the proposed SP-Net can be observed from the heat maps of [Fig.YY] (b). As shown in the figure, the active pillars of SP-Net are initially spread out and form several clusters, in which the ground-truth locations are included. Thanks to dilation effect of sparse convolution, those active pillars can exchange their feature information and strengthen the clusters. At the same time, dynamic pruning of unimportant pillars maintains overall sparsity of the network. As a result, SP-Net can achieve comparable reduction in computation while maintaining the accuracy of the original 3D object detection network ([Table YY]). Such balance between accuracy and sparsity enables SP-Net a promising pillar-base 3D object detection method.


\subsection{Challenges}
\label{subsec:sp-net-challenges}

The main operation of SP-Net is sparse convolution. The major performance bottleneck of sparse convolution is searching for the mapping of sparse input to the output. As discussed earlier, several prior works attempted to optimize the mapping on GPU. In particular, \cite{yan2018second, tang2022torchsparse} have optimized the GPU implementation of sparse convolution algorithms called (SpConv). Still, these hash table-based mapping implementation remains a significant bottleneck, and this issue is even more serious for PointPillars. As a concrete example, we compare the execution time of PointPillars in two ways: 1) Conv2D-based dense pillar processing (PointPillars), and 2) SpConv-based sparse pillar processing (SP-Net). [Table ZZ] shows the latency breakdown on KITTI inference. Although the execution time of SP-Net is smaller thanks to the reduced number of active pillars, its overall execution time is much longer due to long time taken for mapping. 

This observation motivates us to consider a dedicate accelerator for efficiently managing sparse pillars. Prominent prior works have suggested approximate search for mitigating the mapping cost \cite{xu2019tigris,feng2020mesorasi,feng2022crescent} or devised the customized sorting and cache units for expedited search ~\cite{lin2021pointacc}. However, none of these dedicated accelerators have targeted sparse pillar-based 3D object detection, leaving significant room for optimization.  
